Approximate Relational Hoare Logic for Continuous Random Samplings

Approximate relational Hoare logic (apRHL) is a logic for formal verification of the differential privacy of databases written in the programming language pWHILE. Strictly speaking, however, this logic deals only with discrete random samplings. In this paper, we define the graded relational lifting of the subprobabilistic variant of Giry monad, which described differential privacy. We extend the logic apRHL with this graded lifting to deal with continuous random samplings. We give a generic method to give proof rules of apRHL for continuous random samplings.

==> 60endorelational.tex <==
\section{Endorelational apRHL}\label{endorelationalapRHL}
The category $\ERel(\Meas)$ of endorelations on measurable spaces is defined by:
\begin{itemize}
\item An object is a pair $(X,\Phi)$ consisting a measurable space $X$ and a relation $\Phi$ on $X$.
\item An arrow $f \colon (X,\Phi) \to (X',\Phi')$ is $f \colon X \to X'$ in $\Meas$ such that $(f \times f)(\Phi) \subseteq \Phi'$.
\end{itemize}
We then introduce the $M$-graded monad $\{{\mathcal{G}'}^{(\gamma,\delta)}\}_{(\gamma,\delta) \in M}$ on $\ERel(\Meas)$ that captures the notion of differential privacy as follows: for each relation $\Phi$ on $X$,
\begin{align*}
	{\mathcal{G}'}^{(\gamma,\delta)} \Phi
%	\\
%	& = \SetBraket{
%		(\nu_1,\nu_2) \in \mathcal{G}X \times \mathcal{G}X
%		| \forall{ f \colon \Phi \to \leq \text{ in } \ERel(\Meas)}.
%			\int_X f~d\nu_1 \leq \varepsilon \int_X f~d\nu_2 + \delta
%	}
%	\\
	& = \SetBraket{
		(\nu_1,\nu_2) \in \mathcal{G}X \times \mathcal{G}X
		| \forall{A \in \Sigma_X}.
			\Phi(A)\subseteq A \implies \nu_1(A) \leq \varepsilon \nu_2(A) + \delta
	}.
\end{align*}
We now introduce the endorelational variant of (measurable) apRHL.
The judgement of apRHL is changed to:
\[
	c \sim_{\gamma, \delta} c \colon \Psi \Rightarrow \Phi
\]
where $c$ is a command, and $\Psi$ and $\Phi$ are precondition and postcondition respectively.
The validity is changed to:
\[
	\models c \sim_{\gamma, \delta} c \colon \Psi \Rightarrow \Phi
	\iff
	\interpret{\Gamma\vdash c} \colon \Psi \to \overline{\mathcal{G}'}^{(\gamma, \delta)} \Phi \text{ in }\ERel(\Meas)
\]
where
$
	\overline{\mathcal{G}'}^{(\gamma, \delta)}
	= ({\mathcal{G}'}_{(\gamma, \delta)}\wedge \opposite{({\mathcal{G}'}_{(\gamma, \delta)}\opposite{(-)})})
$.
The all proof rules of the endorelational apRHL except [comp] are inherited from the original one.

In the [comp] rule, the requirement of measurability of the postconditions is changed to the reflexivity of the postconditions.
Thus the [comp] rule in the endorelational apRHL is given as follows:
\[
	\AxiomC{$
		\begin{array}{l@{}}
			\mathrm{Eq}_{\interpret{\Gamma}} \subseteq \Phi, \Phi'\\
			\models c \sim_{\gamma,\delta} c \colon \Psi \Rightarrow \Phi \\
			\models c \sim_{\gamma',\delta'} c \colon \Psi' \Rightarrow \Phi'
		\end{array}
	$}
	\RightLabel{{[comp]}}
	\UnaryInfC{$
			\models c \sim_{\gamma\gamma',\min(\delta+\gamma\delta',\delta'+\gamma'\delta)} c \colon \Psi\circ\Psi' \Rightarrow \Phi\circ\Phi' 
	$}
	\DisplayProof.
\]
The soundness of proof rules of endorelational apRHL is proved in the same or easier way as the original one.
